Radio Counterpart Candidates to 4FGL-DR2 Unassociated Sources

For the duration of the Fermi Gamma-Ray Space Telescope's mission, approximately one-third of the point sources detected have been noted as "unassociated," meaning that they seem to have no known counterpart at any other wavelength/frequency. This mysterious part of the gamma-ray sky is perhaps one of the largest unknowns in current astronomical pursuits, and as such has been probed extensively by various techniques at various frequencies. Radio frequencies have been perhaps one of the most fruitful, producing a large fraction of the identified and associated Active Galactic Nuclei (AGN) and pulsars noted in each update of the point source catalogs. Here we present a catalog of 7432 radio counterpart candidates for unassociated gamma-ray fields in the 2nd Data Release of the 4th Fermi Point Source Catalog (4FGL-DR2). A description of the catalog and source types is provided followed by a discussion that demonstrates how the results of this work will aid new associations and identifications. As part of this work, we also present a first catalog derived from "quicklook" images of the Very Large Array Sky Survey (VLASS).

==> refs/manual_refs.tex <==
\bibitem[Hagberg et al. (2008)]{SciPyProceedings_11} Hagberg, A.~A., Schult, D.~A., Swart, P.~J., \ Proceedings of the 7th Python in Science Conference
